A Qualitative and Quantitative Analysis of Container Engines

Containerization is a virtualization technique that allows one to create and run executables consistently on any infrastructure. Compared to virtual machines, containers are lighter since they do not bundle a (guest) operating system but they share its kernel, and they only include the files, libraries, and dependencies that are required to properly execute a process. In the past few years, multiple container engines (i.e., tools for configuring, executing, and managing containers) have been developed ranging from some that are ``general purpose'', and mostly employed for Cloud executions, to others that are built for specific contexts, namely Internet of Things and High-Performance Computing. Given the importance of this technology for many practitioners and researchers, this paper analyses six state-of-the-art container engines and compares them through a comprehensive study of their characteristics and performance. The results are organized around 10 findings that aim to help the readers understand the differences among the technologies and help them choose the best approach for their needs.

==> 4-features-backup.tex <==
%In the following, we first present each container engine along with their main functionalities, and then we compare them in Section~\ref{sec:qualitative-disc}.

All six container engines are open source and their development is active. Most of the implementations are written in Go, but Charliecloud and Sarus: the former is written using a mix of shell scripts and C code, the latter is written in C++. Even if we have identified three groups, each solution, with the exception of balenaEngine that requires a dedicated OS, can be used in any context due to the natural portability of containers (at least on Linux-based systems). 



All six container engines  support the Open Container Initiative (OCI, \cite{oci_website}), either fully or partially, which was established in 2015 to standardize container technology. The main parts of the standard so far are: \textit{image-spec}~\cite{ociimage_website}, for image creation, and \textit{runtime-spec}~\cite{ociruntime_website}, for container execution.

\subsection{Docker}
\luc{circa 50 righe}

Docker was the first popular engine, and it is still probably the most famous one. It provides a complete production platform for developing, distributing, securing, and orchestrating container-based solutions. It is easy to use, well established among developers, and its general-purpose nature fits almost any software project. It uses the features of the Linux Kernel, like namespaces and control groups, to package an application on a development machine (e.g., a laptop), and run it unmodified on any public cloud, private cloud, or even on bare metal node, where the Docker Engine is installed. Docker exploits \textit{containerd}~\cite{containerd_website} for managing and running containers, which in turn uses \textit{run-c}~\cite{runc_website} (developed in the context of OCI) as low-level container runtime for container creation.

Docker images can be built from a Git repository, from a compressed archive, or a Dockerfile. A Dockerfile is a text file that defines all the commands needed to build an image.  A Docker image consists of several read-only layers of data, each of them corresponding to a Dockerfile instruction. The layers are stacked and contain only the changes from the previous one. Layered images are particularly useful because they allow reusing any layer as starting point for a different image. Being read-only, the layers shared across different images are only stored once on the disk, and if needed, in memory. 

When a new container instance is created from an image, a writable layer, called the container layer, is also created on top of the image layers. This layer hosts all changes made to the running container, for example, it stores newly written files, modifications to existing files, and deleted files to allow for customizing the container. Changes made to the container layer do not affect image layers.

Docker allows one to publish images onto private or public \textit{registries} that act as shared repositories, where images can be versioned through tags. This way, different versions of the same image (e.g., latest, old or beta version) can be associated with the same project.
Docker also provides a public, official registry, called \textit{Docker Hub}~\cite{docker_hub_website}, that offers a rich set of base images that can be used as a starting point for building new containerized applications. \textit{Docker Registry} allows us to create private registries. 

Besides creating, running, pausing, stopping, and deleting single containers, \textit{Docker Compose} allows us to configure and run multi-container applications. Users write \textit{docker-compose} files to define all container images used by the application, and the instances we need of each image. Typical use cases are ``traditional'' three-tier applications or microservices where a single system is composed of multiple separated components (i.e., multiple executables). By default, Docker Compose also sets up a network for the application, and each container is reachable by the others.

\textit{Docker Swarm} lets users manage containers deployed across multiple machines \luc{docker compose no?}. It uses the standard Docker API and networking for merging a pool of Docker hosts into a virtual, single host. It also provides means to scale applications or single containers that can be replicated onto Swarm nodes. \luc{Cosa sono gli Swarm nodes?}

Docker is a client-server application. The server is the Docker daemon (\textit{dockerd}) that processes the requests sent by clients through a command-line interface (CLI) or a RESTful API and manages Docker images and instances. The daemon is executed with root privileges, and thus only trusted users should be allowed to control the daemon. A \textit{rootless} mode was available as an experimental feature starting from version $19.03$ and it has been fully supported since version $20.10$. \luc{Non ho capito: servono i privilegi di root o no?} Note that it is also possible to run Docker without root permissions by creating a dedicated user group. However, this group must have a set of permissions equivalent to the one of a root user. The rootless mode executes the Docker daemon and containers inside an isolated user namespace (a feature that Docker itself uses also to isolate containers with one another). Thus, both the daemon and the containers run without root privileges. By default, Docker starts containers with a restricted set of Linux kernel capabilities \cite{kernelcap_website}\cite{linuxcap_paper} to allow us to implement a fine-grained access control system. The best practice is to remove all the capabilities except those explicitly required by the application.
\luc{Non ho capito. L'ultima parte sui permessi mi sembra abbastanza arrotolata. Serve essere root o no? Il controllo degli accessi come si innesta?}

\subsection{Podman}

\luc{Circa 28 righe}

Podman~\cite{gantikow2020rootless} is younger compared to Docker and is a container engine used for developing, managing, and running OCI containers and container images. It is based on library \textit{libpod}, from the same developers, that is used for managing the entire container lifecycle. It uses, like Docker, the \textit{run-c} container runtime for instantiating containers.

Podman images are made up of multiple layers as in Docker, and they can be built from a Dockerfile or from a so-called \textit{Containerfile} (same syntax as Dockerfiles but with a different file extension). At its core, Podman uses Buildah~\cite{buildah_website} to build container images. Since it replicates all the commands we can find in a Dockerfile, Podman allows the user to build images with or without Dockerfiles while not requiring any root privileges. Podman supports both OCI and Docker image, and allows one to pull images from a local directory that stores all the image files, a Docker registry, or an OCI archive, that is, an image that complies with OCI. 

Similarly to Docker, Podman exploits \textit{cgroups}~\cite{cgroups}, a feature of the Linux kernel, for allocating resources to containers. It provides a mechanism to limit and monitor system resources like CPU time, system memory, disk bandwidth, and network bandwidth. If the container is executed in rootless mode, \textit{cgroup v2} is required.

Podman provides a rich set of commands to maintain and modify OCI container images and to manage the entire container lifecycle. It uses an interface that is compatible with the Docker's one, but for orchestrating containers, it relies on external tools such as Kubernetes~\cite{k8s_website}. Podman can automatically generate Kubernetes configuration files and allows, starting from version 3.0, to convert Docker Compose files into Kubernetes ones.

Podman is daemonless and so it has no background service and the container runtime is executed only when requested. This way, Podman offers less attack surface, because it is not always in execution. It does not require root privileges by leveraging, like Docker, user namespaces. Both Docker and Podman require an initial configuration by a system administrator to enable rootless execution. 
Podman allows us to sign images to only trust selected image providers. Moreover, to mitigate man-in-the-middle attacks, the image can be signed with a GNU Privacy Guard (GPG) key before pushing it to a remote registry. In this configuration, all the nodes running Podman must be properly configured to retrieve the signatures from a remote server.

\subsection{Charliecloud}

\luc{19 righe di cui 15 circa di sicurezza}

Charliecloud~\cite{charliecloud_website,charliecloud_paper1,charliecloud_paper2} focuses on the management of containers on HPC frameworks by simplifying the packaging and transmission of HPC applications, and is the lightest solution among the analyzed ones (i.e., only a few thousands of LOC). Charliecloud supports the OCI runtime, even though it is an experimental and partial feature\footnote{ \url{https://hpc.github.io/charliecloud/command-usage.html\#ch-run-oci}}.

For image creation, Charliecloud uses external builders ---including Docker and Buildah---, or an internal one, called \textit{ch-image}. The image can be built with or without privileges, depending on the used builder. The created image is wrapped with a Charliecloud interface and converted into a compressed archive that can be easily moved on the HPC cluster. The archive is then unpacked and executed without root privileges. 

Charliecloud provides a command to inject files into a container on a specific host with ad-hoc parameters for GPU configuration and MPI. However, this command is still an experimental feature. \luc{Non ho capito il senso della frase precedente}

Charliecloud only needs Linux user namespaces to run containers without the need of any privileged operations. It is daemonless and requires only minimal configuration changes on the computing center. It is not designed to be an isolation layer, so containers have full access to host resources. Charliecloud commands require privileged access only when used along with external builders such as Docker. 
This approach avoids most security risks while maintaining access to the performance and functionality already offered~\cite{charliecloud_paper1} since image building is executed on the user machine and not in the HPC center. \luc{non ho capito l'ultima frase} 

\subsection{Singularity}

\luc{39 righe}

Singularity~\cite{singularity_paper1,singularity_paper2,singularity_paper3} is a container engine optimized for the computation of HPC workloads. It can also be used in cloud deployments and supports Docker images and registries. From version 3.1.0, Singularity is fully OCI compliant, and supports both OCI specifications: image-spec and runtime-spec.

Singularity allows us to build containers from external resources, as its official public registry, called \textit{Singularity Cloud Library}~\cite{singularity_cloud_library_website} (SIC), and Docker Hub, converted and used in Singularity \luc{Se sono solo questi due, possiamo dirlo esplicitamente}. Singularity Definition Files (SDF), similarly to Dockerfiles, are used to create container images. An SDF is composed of two parts, the \textit{header}, which defines the configuration of the execution environment (e.g., kernel features, Linux distribution), and \textit{sections}, which execute commands during the build process. The container can be produced in two different formats: a writable sandbox for interactive development, or in the Singularity Image Format (SIF), a compressed read-only format that can be easily moved, shared, and distributed. To optimize image size, Singularity builds images using SquashFS~\cite{squashfs_website}, a compressed read-only filesystem.

Singularity provides two execution models: \textit{hybrid} and \textit{bind}. The former allows one to exploit both the MPI implementations provided by the host and the one inside the containers, increasing the overall portability of the container \luc{Non ho capito la frase precedente, ma MPI dovrebbe essere enfatizzato per tutte le soluzioni HPC. No?}. The latter uses only the MPI implementation available on the host. Clusters and schedulers such as Torque~\cite{torque}, Slurm Workload Manager~\cite{slurm_website}, and SGE~\cite{sge} are supported by Singularity. It also natively supports  containers that use GPU frameworks such as NVIDIA CUDA\footnote{\url{https://developer.nvidia.com/cuda-toolkit}} and AMD ROCm\footnote{\url{https://rocmdocs.amd.com/en/latest/}}. The user can exploit GPUs within containers as long as the host operating system has the proper driver installed. Singularity supports both OpenMPI\footnote{\url{https://www.open-mpi.org}} and MPICH\footnote{\url{https://www.mpich.org}}, two popular implementations of MPI. \luc{Ma non andava detto prima?}

Singularity containers can be signed and verified using PGP keys and thus provide a trusted method to share containers. Singularity supports the encryption/decryption of containers at runtime to create a secure and confidential container environment. Singularity does not provide the layer mechanism offered by Docker, thus the container is always built from scratch and it is not possible to reuse layers to speed up the building process. It also allows us to build containers without root privileges by using a \textit{fakeroot} feature, but it must be configured to work.

Singularity requires containers to have the same permissions as the users that started them, while the access to files within the container runtime is managed by the standard POSIX permissions. Containers are started with flag $PR\_NO\_NEW\_PRIVS$ that prevents applications to gain additional privileges. On multi-user, shared systems, such as HPC centers, Singularity allows an unprivileged user to run a container as root with  \textit{FakeRoot}\footnote{\url{https://wiki.debian.org/FakeRoot}}. \luc{Ma non lo abbiamo gi\`a detto sopra?} This way, the user has almost the same administrative rights as root but only within the container. In addition, Singularity provides several strategies to ensure safety in these types of environments. \luc{Csa vuol dire?} Singularity is daemonless and containers can be launched in the background as \textit{detached} containers \luc{E cosa vuol dire?}. It is possible to install Singularity without a root user even if some limitations apply. \luc{Magari da anticipare sopra quando parliamo di permessi}

\subsection{Sarus}

\luc{17 righe}

Sarus~\cite{sarus_website,sarus_paper} is the most recent project, with the lowest number of releases, and has been designed to run containers in the HPC context. It leverages the OCI standard, and run-c \cite{runc_website} as container runtime, and provides an extensible runtime to support current and future custom hardware while achieving native performance. 

Sarus does not manage image creation or publication, but an image can be loaded from a local tar file or registry, including Docker or OCI-compliant ones. Once the image layers are downloaded, they are uncompressed in a temporary directory. The layers are then compressed together using  SquashFS (as in Singularity). This compression improves the I/O performance of the container and reduces the size of the image on the disk. 

Sarus supports and integrates the Slurm Workload Manager. GPU devices are supported through a dedicated library, namely, the NVIDIA Container Runtime \cite{nvidiacontainer_website}  (that is OCI-compatible). It also allows swapping MPICH-based MPI implementations inside a container with an ABI-compatible~\cite{abi_website} library running in the host to increase performance.  Moreover, Sarus provides support for parallel file systems and diskless nodes.

Root permissions are required to install and work with Sarus. For this reason, Sarus checks a list of conditions to ensure that critical files and directories opened during privileged execution meet them.

\subsection{balenaEngine}

\luc{25 righe}

balenaEngine~\cite{balena_website} is based on the Moby Project~\cite{moby_website}, a framework provided by Docker to assemble specialized container systems, and offers a complete platform for deploying IoT applications using OCI-compliant containers. 

Devices must run balenaOS~\cite{balena_os_website}, a Linux-based host operating system customized for the execution of balenaEngine and containers. This operating system, which is compatible with a wide range of computer architectures including armv5, armv6, armv7, aarch64, i386, and x86\_64, is also responsible for running a containerized daemon (device supervisor) that automatically updates running containers if an update is available.

balenaEngine builds Dockerfiles and pulls containers from Docker Hub. When a new version of an image is available, the engine minimizes network bandwidth consumption by only downloading the delta between the image stored on the host device and the updated one.  Atomic image updates make sure that a device cannot end up with a corrupted container. \luc{Perch\'e?}
It also optimizes I/O performance. When a ``standard'' container engine downloads a new image, it first downloads the compressed archive, writes it on the disk, and then extracts it to produce the image. Instead, balenaEngine extracts the files on-the-fly and avoids writing the compressed archive onto the disk.  Preventing page cache thrashing during image download make it work in low-memory situations.

balenaEngine provides multiple security layers. Updates are sent to devices in a reliable and verifiable way to protect devices against attacks. An API key is created for each device, balenaOS then  controls who can access it, the actions that are permitted, and the available communication channels. balenaEngine uses OpenVPN to control the state of its devices. The VPN disallows device-to-device traffic and prohibits outbound traffic to the Internet.
balenaEngine maintains a repository of secured base images \luc{secure o secured?}. Any resource added to these base images is verified by a GPG or a checksum.

\begin{table}[thbp]
	\begin{tabular}{lcccccc}
		\toprule
		  \textbf{Feature} & \textbf{Doc}  & \textbf{Pod} & \textbf{Cha} & \textbf{Sin} & \textbf{Sar} & \textbf{bal} \\
		\midrule
		\multicolumn{7}{c}{\textit{Compatibility}}  \\
		\textit{OCI compliance} & \checkmark & \checkmark
& $\sim$  & \checkmark & \checkmark & \checkmark \\ 
\textit{Support for multiple host operating systems} & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark & $\times$ \\
 \midrule
 \multicolumn{7}{c}{\textit{Image building and usage}}  \\
 \textit{Built-in image builder} & \checkmark & \checkmark
& \checkmark & \checkmark & $\times$ & \checkmark \\
    \textit{Images from Dockerfiles/Containerfiles} & \checkmark & \checkmark
& \checkmark & \checkmark & $\times$ & \checkmark \\  
    \textit{Images from SDFs} & $\times$ \ & $\times$
& $\times$ & \checkmark & $\times$ & $\times$ \\ 
        \textit{Images from git repositories} & \checkmark & \checkmark
& $\times$ & $\times$ & $\times$ & \checkmark \\  
    \textit{Images from archives} & \checkmark & \checkmark
& \checkmark & $\times$ & $\times$ & \checkmark \\  
        \textit{Public/private registries} & \checkmark & \checkmark
& \checkmark & \checkmark & \checkmark & \checkmark \\
        \textit{Support for Docker/OCI images} & \checkmark & \checkmark
& $\sim$ & \checkmark & \checkmark & \checkmark \\
        \textit{Support for SIF} & $\times$ & $\times$
& $\times$ & \checkmark & $\times$ & $\times$ \\
\midrule
 \multicolumn{7}{c}{\textit{Optimizations}}  \\
 \textit{Layered images} & \checkmark & \checkmark
& \checkmark & $\times$ & \checkmark & \checkmark \\
\textit{Differential image updates} & $\times$ & $\times$
& $\times$ & $\times$ & $\times$ & \checkmark \\
\textit{On the fly image extraction} & $\times$ & $\times$
& $\times$ & $\times$ & $\times$ & \checkmark \\
\textit{Image compression} & $\times$ & $\times$
& $\times$ & \checkmark & \checkmark & $\times$ \\ 
\midrule
 \multicolumn{7}{c}{\textit{Containers executions}}  \\
 \textit{Detached executions} &  \checkmark  &  \checkmark 
& $\times$ & \checkmark & $\times$ & \checkmark  \\
\textit{Dynamic Resource Management} & \checkmark & $\times$
& $\times$ & \checkmark & $\times$ & $\times$ \\
\textit{Built-in orchestration capabilities} & \checkmark & $\times$
& $\times$ & $\times$ & $\times$ & \checkmark \\
\textit{Support for workload managers} &  $\times$  &  $\times$ 
 & \checkmark & \checkmark & \checkmark & $\times$  \\
\textit{Support for GPUs} & \checkmark & $\times$
& $\sim$ & \checkmark & \checkmark & \checkmark \\
\textit{Explicit support for MPI libraries} & $\times$ & $\times$
& $\sim$ & \checkmark & \checkmark & $\times$ 
 \\\midrule
  \multicolumn{7}{c}{\textit{Security}}  \\
\textit{Signed container images} & \checkmark & \checkmark
& $\times$ & \checkmark & \checkmark & \checkmark \\
\textit{Rootless executions} & $\sim$ & \checkmark
& \checkmark & \checkmark & $\times$ & $\times$ \\
\textit{Daemonless execution model} & $\times$ & \checkmark
& \checkmark & \checkmark & \checkmark & $\times$ \\
		\bottomrule
	\end{tabular}
	 \caption{Qualitative comparison: \checkmark available, $\sim$ partially available, and $\times$ not available.}
	\label{tab:features}
\end{table}


\subsection{Discussion}
\label{sec:qualitative-disc}

Table~\ref{tab:features} summarises our analysis and organizes discovered features around five main dimensions: i) \textit{compatibility}, the degree of compliance to standards and the availability on different operating systems, ii) \textit{image building and usage}, the ways container engines generate, use, and share container images, iii)  \textit{optimizations}, the techniques employed to reduce resource usage, iv) \textit{container executions}, the features available at runtime, such as resource management and the support to specific libraries and tools, and v) \textit{security}, the way container engines guarantee secure image builds and executions. Note that each technology is abbreviated with the first three letters of their name (e.g., $Doc$ for Docker).

All selected container engines fully support the OCI standard, with the only exception of Charliecloud that only provides it as an experimental feature: the support is only partial and available with a set of additional commands \luc{cosa vuol dire with a set of additional commands?}. OCI assumes that containers be always-on services with a complex lifecycle, while Charliecloud focuses on scientific applications that are usually executed once and are terminated as soon as the required calculations are completed \luc{Non ho capito il problema}. Similarly Singularity provides both OCI-compliant commands (e.g., \textit{singularity oci exec}) and additional ones (e.g., \textit{singularity exec}).

In terms of compatibility, balenaEngine is the only solution that only works on top of balenaOS, a dedicated operating system. This operating system is optimized to run containers on IoT devices, and provides a minimum feature set to avoid saturating them. All other engines can run on full-fledged, standard operating systems.

\vspace{0.5cm}
\begin{mdframed}
\textbf{Finding \#\findings} All analyzed container engines support OCI and standard host operating systems with a few exceptions. Docker, Podman, Sarus, and balenaEngine are fully OCI compliant. Singularity is also compatible with OCI but with a dedicated set of commands, and Charliecloud offers it as an experimental feature. balenaEngine can only run on top of its dedicated oerating system.
\end{mdframed}
\vspace{0.5cm}

\luc{Onestamente questo finding e il testo sopra mi sembrano una ripetizione abbastanza 1 a 1. No?}

All selected container engines, but Sarus, provide means to build images. Docker and Singularity have their own image builder, Podman relies on Buildah, balenaEngine supports Docker, while Charliecloud offers the built-in \textit{ch-image}, Docker, or Buildah.

\luc{Faccio fatica a capire il filo logico della parte che segue tra formato delle immagini, che credevo affrontato sopra, dokerfile o simili, repositories}

Dockerfiles (i.e., Containerfiles) are supported by all the engines (again, but Sarus), while only Singularity comes with a proprietary SDF format.
Docker, Podman, and balenaEngine \luc{also, \`e una aggiunta a Dockerfiles?} provide support for building images from either git repositories or archive files (e.g., tar files).

Docker uses its image format (that is the base for the OCI specification) and supports registries to access container images from different execution environments. It provides an official public registry, DockerHub, to ease image sharing. Podman supports any standardized OCI image (including Docker ones) and supports Docker-compatible registries. \luc{Non ho capito il riferimento a OCI qui e quanto diciamo sopra, ovvero che tutti sono compatibili} 

Charliecloud images can be pulled from DockerHub, other Docker-compatible registries, and archives. \luc{Ma non lo abbiamo gi\`a detto sopra?}
Singularity supports Docker/OCI images along with proprietary SIF, ones which are not supported by any other engine. Similarly to Docker, Singularity provides a public registry to share container images and also supports Docker ones. \luc{Mi sono perso. OCI \`e il formato dell'immagine? Se s\`i, non dovrebbe essere parte di quanto abbiamo detto sopra, dove non parliamo di SIF?}

Sarus supports already-built images that are OCI compliant, and that can be downloaded from public and private registries. \luc{Di che tipo?}
balenaEngine uses Docker behind-the-scene for both image building and usage providing analogous capabilities. \luc{Ma non lo abbiamo gi\`a detto sopra?}

\vspace{0.5cm}
\begin{mdframed}
\textbf{Finding \#\findings.} All analyzed engines but Sarus provide means to build images from Dockerfiles/Containerfiles. Singularity can also use a proprietary format for both image definition and building. Non-HPC engines support images created from git repositories and archives \luc{C'\`e una ragione? La tabella per\`o dice qualcosa di leggermente diverso}, while all the engines allow users to share and download images using private or public registries. Charliecloud supports images loaded from archives (i.e., tarballs). \luc{Ma non \`e uguale a creare immagini da archivi, come detto sopra}
\end{mdframed}
\vspace{0.5cm}

%%%%%%%%%%%%%%%%%%%%%%

All engines provide key optimizations. All but Singularity exploit layered images, an approach pioneered by Docker. This way, different images can share common files and components without the need of storing them multiple times. 
balenaEngine is built to optimize the usage of network and I/O bandwidth. When an image is updated, the devices are notified and only the differences are downloaded, and in case of faults (e.g., out of batteries) container images cannot be corrupted \luc{Perch\'e? Non abbiamo già detto qualcosa di simile}. When working with container images to be generated from archives, balenaEngine builds the image while uncompressing the files without the need for occupying the disk with temporary files. During the extraction, balenaEngine also reduces the memory footprint by limiting page caching.

Sarus does not provide any built-in mechanism for image creation and publication but optimizes existing images (e.g., Docker or OCI ones) by reducing their size through SquashFS, an optimization that is also employed by Singularity.

\vspace{0.5cm}
\begin{mdframed}
\textbf{Finding \#\findings.} Layered images are a widespread technique to save disk space by allowing images to share common parts. balenaEngine provides some key optimizations to reduce network transfers (i.e., differential image updates) and disk usage (i.e., on-the-fly image extraction). Sarus and Singularity compress images with SquashFS to reduce disk usage.
\end{mdframed}
\vspace{0.5cm}

When it comes to container executions, one of the main features is the support for ``detached'' executions, that is, the ability to run long-lasting interactive processes (e.g., a database management system or a web server). While applications executed in the cloud or IoT infrastructures may benefit from this feature, HPC applications are usually non-interactive and terminate as soon as the calculations are completed. For this reason, Charliecloud and Sarus do not support detached executions by design. \luc{E singularity?}

While all container engines provide the means to allocate resources (e.g., cores) to a container at startup time, only Docker and Singularity allow for dynamic resource management, that is, the reconfiguration of allocated resources at runtime.

GPU computations are supported by all the engines, but Podman. Charliecloud provides this feature but requires non-trivial effort\footnote{\url{https://hpc.github.io/charliecloud/command-usage.html\#notes}} (e.g., recompilation) to configure some important GPU-related libraries (e.g., NVIDIA ones). \luc{Come si spostano le GPU e balena?}

balenaEngine provides some important orchestration capabilities to deploy and update containers on a fleet of registered IoT devices, while Docker provides two dedicated tools: Docker Compose, to create blueprints of applications that use multiple container images (e.g., an application server connected to a database), and Docker Swarm, to orchestrate containers running on multiple machines. Instead, Podman relies on external tools and provides built-in integration with Kubernetes \luc{Docker no?}. HPC engines do not provide ad-hoc orchestration capabilities but they support MPI libraries that help developers write complex distributed computations, and workload managers that oversee distributed executions. \luc{Non ho capito l'ultima parte. Perch\'e MPI si confronta con Kubernetes? Kubernetes non \`e anche un workload manager?}

%%%%%%%%%%%%%%%%%

In particular, Singularity eases the operations to execute containers on the HPC data center by supporting natively most of the available schedulers and letting containers use an underlying MPI installation on the host OS or one that is enclosed in the container.  Sarus and Charliecloud support Slurm as workload manager. The former also supports MPI libraries and their different implementations, while the latter requires the aforementioned extra configuration steps.

\vspace{0.5cm}
\begin{mdframed}
\textbf{Finding \#\findings.} Detached executions are not supported by Charliecloud and Sarus because of their focus on scientific applications. Docker and Singularity provide means to dynamically allocate resources, while only Docker and balenaEngines have built-in orchestration capabilities. HPC engines provide ad-hoc support for workload managers, GPU executions, and MPI-based computations.
\end{mdframed}
\vspace{0.5cm}


Docker and balenaEngine support signed container images and have a daemon-based architecture, and by default, the daemon is executed with root privileges which can harm the security of the system. Only recent versions of Docker support rootless executions.
Podman does not use a daemon and it is only executed when needed increasing the overall security. As Docker, Podman supports signing container images before pushing them to a registry.   

To enhance security, Singularity is daemonless and restricts the permissions available in a container instance to the ones owned by the users that launched it. No additional privileges can be gained. \textit{FakeRoot} allows having containers with administrative rights in a safe way. 

Charliecloud is daemonless but does not provide the same level of isolation as other runtimes. However, it only requires root access for user-based operations (image creation), while the execution on the HPC data center can be unprivileged unless the application itself requires more permissions. 
Sarus is also daemonless. It requires root permissions for multiple operations but checks that proper restrictions are met at runtime. Both Charliecloud and Sarus support image signing. 


\vspace{0.5cm}
\begin{mdframed}
\textbf{Finding \#\findings.} All container engines except for Singularity support container image signing to increase reliability. Rootless executions are supported by Podman, Charliecloud, Singularity, and only recently by Docker. Docker and balenaEngine share the same daemon-based architecture, while the others are daemonless.
\end{mdframed}




==> 6_hpc-old.tex <==
The last set of experiments is dedicated to evaluating the performance of HPC-specific container engines. In particular, the goal of the tests is to analyze the overhead introduced during the execution of computationally intensive and highly parallel applications. 

\subsection{Experiment Setup}
\label{hpc:cluster_setup}

We deployed a cluster of high-performance virtual machines on Microsoft Azure. We used machines of type HB60rs equipped with 60 cores and 240GB of RAM. These machines also feature a network interface for RDMA (remote direct memory access) connectivity that allows processes to communicate over an InfiniBand network (100 Gb/sec Mellanox EDR with single root input/output virtualization). For the experiments, we used up to 8 instances of HR60rs VMs.

We initially used Azure Cyclecloud, a tool provided by Microsoft, for the configuration of HPC clusters.
Since the tool was quite unstable and slow, we created a set of Ansible playbooks~\footnote{\url{https://github.com/deib-polimi/containers-SlurmCluster}} to automate the management operations. We set up the cluster with the Slurm workload manager and a distributed file system (NFS\footnote{\url{http://nfs.sourceforge.net}}). We used the Azure CentOS VM image since it was designed for HPC applications and embeds all the necessary drivers to work with InfiniBand and MPI. We used OpenMPI 4, configured in \textit{hybrid} mode so that both the library installed in the host node and the one in the container can be used (see Section~\ref{sec-features}).

% docker
We built the container images with Docker to use the same solution across the different engines. We created a Dockerfile\footnote{\url{https://github.com/deib-polimi/containers-DockerHPC}}, starting from the one provided by Azure\footnote{\url{https://github.com/Azure/batch-shipyard/tree/master/recipes/mpiBench-Infiniband-OpenMPI}} that includes support for InfiniBand and OpenMPI. In addition, we updated the drivers to match the one installed on the host VM and we included the benchmarks we wanted to execute.
We used two well-known test suites for MPI: the OSU Micro-Benchmarks\footnote{\url{http://mvapich.cse.ohio-state.edu/benchmarks/}}  by the Ohio State University, and mpiBench\footnote{\url{https://github.com/LLNL/mpiBench}} by the Lawrence Livermore National Laboratory. 

While we successfully configured both Singularity and Charliecloud, we could not make Sarus properly execute the benchmarks by using the envisaged OpenMPI tools. However, the team behind Sarus executed some of the benchmarks we used on its own, and the results are publicly available~\cite{sarusosu}.

We run three types of experiments: \textit{latency}, \textit{all-to-all}, and \textit{scatter/gather}. The first two are part of the OSU benchmark, while the third is included in mpiBench. Test \textit{latency} measures the min, max, and average latency of a ping-pong communication between two processes. The messages are sent repeatedly with different payload sizes to measure one-way latency. Test \textit{all-to-all} measures the min, max, and average latency of the $MPI\_Alltoall$ operation in which each  node sends (receives) a message to (from) all the other nodes, among \textit{all} involved processes.  Finally, test \textit{scatter/gather} measures the latency of sending messages (between 0 and 64kB) through the MPI primitives \textit{scatter} and \textit{gather}. 
To automate the execution of these benchmarks with Slurm, we developed a set of scripts\footnote{\url{https://github.com/deib-polimi/containers-MPIBenchmarksBatch}}. The container images were fetched from local disks to avoid any performance degradation due to network overhead.

\subsection{Results}
\label{hpc:results_osu}

\begin{figure}[t]
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_latency_operation_2_nodes_1_cores.pdf} 
        \caption{Test \textit{latency} - 2 nodes - 1 core}
        \label{fig:osu_latency_2nodes_1c}
    \end{subfigure}
    % \begin{subfigure}{0.38\textwidth}
    %     \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_latency_operation_1_nodes_2_cores.pdf} 
    %     \caption{1 nodes - 2 cores}
    %     \label{fig:osu_latency_1node_2c}
    % \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_7_nodes_30_cores.pdf}
        \caption{Test \textit{all-to-all} - 7 nodes}
        \label{fig:osu_alltoall_7nodes_30c}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_30_cores_64_size.pdf} 
        \caption{Test \textit{all-to-all} - 64 bytes}
        \label{fig:osu_alltoall_64_30c}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_30_cores_65536_size.pdf}
        \caption{Test \textit{all-to-all} - 65 kB}
        \label{fig:osu_alltoall_65kb_30c}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_7_nodes_60_cores.pdf}
        \caption{Test \textit{scatter} - 7 nodes}
        \label{fig:mpibench_scatter_7nodes_60c}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_7_nodes_60_cores.pdf}
        \caption{Test \textit{gather} - 7 nodes}
        \label{fig:mpibench_gather_7nodes_60c}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_60_cores_64_bytes.pdf} 
        \caption{Test \textit{gather} - 64 bytes}
        \label{fig:mpibench_gather_64bytes_60c}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_60_cores_65536_bytes.pdf}
        \caption{Test \textit{gather} - 65 kB}
        \label{fig:mpibench_gather_65kb_60c}
    \end{subfigure}
    \caption{\blue{MPI experiments}.}
    \label{fig:osu_latency_size}
\end{figure}

% osu latency
Figure~\ref{fig:osu_latency_size} shows the results for test \textit{latency}. The charts show how the message size (from 1 byte to 4MB) affects the operation time (reported in $\mu s$) during the execution with no containers, (\textit{nocont}), Singularity, and Charliecloud. We report the data obtained with 2 nodes and 1 core each (Figure~\ref{fig:osu_latency_2nodes_1c}) and a single node with 2 cores (Figure \ref{fig:osu_latency_1node_2c}). Since the results clearly show there is no significant difference among the different executions, the overhead introduced by container engines is negligible. 

% \begin{figure}[t]
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_2_nodes_30_cores.pdf} 
%         \caption{2 nodes}
%         \label{fig:osu_alltoall_2nodes_30c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_4_nodes_30_cores.pdf} 
%         \caption{4 nodes}
%         \label{fig:osu_alltoall_4nodes_30c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_7_nodes_30_cores.pdf}
%         \caption{7 nodes}
%         \label{fig:osu_alltoall_7nodes_30c}
%     \end{subfigure}
%     \caption{Test \textit{all-toall} - Cluster size.}
%     \label{fig:osu_alltoall_nodes_30c}
% \end{figure}

% osu alltoall
Figure \ref{fig:osu_alltoall_nodes_30c} shows the results for test \textit{all-to-all} with 30 cores per node (leaving half of the computational capacity to process incoming messages), three cluster configurations (2, 4 and 7 nodes), and a variable message size (from 0 to 4MB). All the charts show the average latency in $\mu s$.
Charliecloud and Singularity perform very similarly in all the experiments. When using 2 nodes (Figure \ref{fig:osu_alltoall_2nodes_30c}), the latency is around 2 times greater than with containers with a message size between 0 and 512 bytes. For larger sizes, the overhead introduced is almost negligible. Similar results are obtained with 4 (Figure \ref{fig:osu_alltoall_4nodes_30c}) and 7 nodes (Figure \ref{fig:osu_alltoall_7nodes_30c}) with a significant overhead when operating with small message sizes. 

% \begin{figure}[htbp]
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_30_cores_8_size.pdf} 
%         \caption{8 bytes}
%         \label{fig:osu_alltoall_8_30c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_30_cores_64_size.pdf} 
%         \caption{64 bytes}
%         \label{fig:osu_alltoall_64_30c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/osu_alltoall_operation_30_cores_65536_size.pdf}
%         \caption{65 kB}
%         \label{fig:osu_alltoall_65kb_30c}
%     \end{subfigure}
%     \caption{Test \textit{all-toall} - Message size.}
%     \label{fig:osu_alltoall_size_30c}
% \end{figure}

Figure~\ref{fig:osu_alltoall_size_30c} shows the results for test \textit{all-to-all} with 30 cores per node, a fixed message size (either 8, 16 bytes or 65kB), and a variable number of nodes. The overhead does not appear to be strongly correlated with the number of nodes in the system. In the experiment with 8 byte messages (Figure \ref{fig:osu_alltoall_8_30c}) the latency introduced by container engines ranges from 1.2 to 2 times the one with no containers (\textit{nocont}); similar values were obtained with 64 bytes (Fig. \ref{fig:osu_alltoall_64_30c}). With 65kb messages, Figure ~\ref{fig:osu_alltoall_65kb_30c}, the overhead is negligible with more than two nodes.

All these experiments suggest that container engines introduce significant overheads with (very) small messages, while it becomes negligible when the size increases (if more than one node is employed). 


% \begin{figure}[htbp]
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_2_nodes_60_cores.pdf} 
%         \caption{2 nodes}
%         \label{fig:mpibench_scatter_2nodes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_4_nodes_60_cores.pdf} 
%         \caption{4 nodes}
%         \label{fig:mpibench_scatter_4nodes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_7_nodes_60_cores.pdf}
%         \caption{7 nodes}
%         \label{fig:mpibench_scatter_7nodes_60c}
%     \end{subfigure}
%     \caption{Test \textit{scatter} - Cluster size.}
%     \label{fig:mpibench_scatter_nodes_60c}
% \end{figure}

% \begin{figure}[htbp]
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_2_nodes_60_cores.pdf} 
%         \caption{2 nodes}
%         \label{fig:mpibench_gather_2nodes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_4_nodes_60_cores.pdf} 
%         \caption{4 nodes}
%         \label{fig:mpibench_gather_4nodes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_7_nodes_60_cores.pdf}
%         \caption{7 nodes}
%         \label{fig:mpibench_gather_7nodes_60c}
%     \end{subfigure}
%     \caption{Test \textit{gather} - Cluster size.}
%     \label{fig:mpibench_gather_nodes_60c}
% \end{figure}



Figures~\ref{fig:mpibench_scatter_nodes_60c} and~\ref{fig:mpibench_gather_nodes_60c} show the results obtained for tests \textit{scatter/gather} with 60 cores per node, three cluster configurations (2, 4 and 7 nodes), and a variable message size (from 0KB to 100KB). All the charts show the average latency in $\mu s$.

Obtained results confirm the previous ones. Charliecloud and Singularity appear to have similar performance and they only introduce overhead with small messages. For example, the two engines added a latency that ranges between 1.3 to 5 times the execution with no container when the message size is between 0 and 256 bytes and we execute \textit{scatter} operations; the overhead becomes negligible with bigger messages. The results obtained with \textit{gather} operations are similar but with a smaller maximum overhead.

% \begin{figure}[htbp]
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_60_cores_8_bytes.pdf} 
%         \caption{8 bytes}
%         \label{fig:mpibench_scatter_8bytes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_60_cores_64_bytes.pdf} 
%         \caption{64 bytes}
%         \label{fig:mpibench_scatter_64bytes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Scatter_operation_60_cores_65536_bytes.pdf}
%         \caption{65 kB}
%         \label{fig:mpibench_scatter_65kb_60c}
%     \end{subfigure}
%     \caption{Test \textit{scatter} - Message size.}
%     \label{fig:mpibench_scatter_size_30c}
% \end{figure}

% \begin{figure}[htbp]
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_60_cores_8_bytes.pdf} 
%         \caption{8 bytes}
%         \label{fig:mpibench_gather_8bytes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_60_cores_64_bytes.pdf} 
%         \caption{64 bytes}
%         \label{fig:mpibench_gather_64bytes_60c}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth, trim={0 0 0 2cm},clip]{graphs/mpi/mpibench_Gather_operation_60_cores_65536_bytes.pdf}
%         \caption{65 kB}
%         \label{fig:mpibench_gather_65kb_60c}
%     \end{subfigure}
%     \caption{Test \textit{gather} - Message size.}
%     \label{fig:mpibench_gather_size_30c}
% \end{figure}

This behavior is even clearer when fixing message sizes (either 8, 16 bytes or 65kB) and varying the number of nodes (Figures ~\ref{fig:mpibench_scatter_size_30c} and~\ref{fig:mpibench_gather_size_30c}). As with test \textit{all-to-all}, the overhead is almost constant and quite significant with the first two configurations, while with messages of 65kB,  the overhead becomes negligible.

\vspace{0.5cm}
\begin{mdframed}
\textbf{Finding \#\findings.} Container engines dedicated to HPC obtained almost identical performance compared to executions without containers in tests that involved simple MPI communications. When tested with more complex operations, the overhead is still negligible unless the messages exchanged are small (less than 0.5MB).
\end{mdframed}




